Divide-and-conquer variational quantum algorithms for large-scale electronic structure simulations

Exploring the potential application of quantum computers in material design and drug discovery has attracted a lot of interest in the age of quantum computing. However, the quantum resource requirement for solving practical electronic structure problems are far beyond the capacity of near-term quantum devices. In this work, we integrate the divide-and-conquer (DC) approaches into the variational quantum eigensolver (VQE) for large-scale quantum computational chemistry simulations. Two popular divide-and-conquer schemes, including many-body expansion~(MBE) fragmentation theory and density matrix embedding theory~(DMET), are employed to divide complicated problems into many small parts that are easy to implement on near-term quantum computers. Pilot applications of these methods to systems consisting of tens of atoms are performed with adaptive VQE algorithms. This work should encourage further studies of using the philosophy of DC to solve electronic structure problems on quantum computers.

==> Makefile <==
base_name := manuscript
datestamp := $(shell date +"%Y-%m-%d")
workdir   := $(shell basename $(shell pwd))


%.pdf: %.tex
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<
	bibtex $*.aux
	pdflatex --interaction=nonstopmode $<
	pdflatex --interaction=nonstopmode $<




all: $(base_name).pdf  
	(evince $(base_name).pdf  &)


$(base_name).pdf: $(base_name).tex $(base_name).bib 

figures:
	$(MAKE) -C figures

dated:
	[ ! -d archive ] && mkdir archive
	$(MAKE) pdf
	cp -a $(base_name).pdf archive/$(base_name)-$(datestamp).pdf

tgz:
	$(MAKE) clean
	cd .. && tar -zcvf $(base_name)-$(datestamp).tgz $(workdir)

backup:
	$(MAKE) tgz
	cd .. && rsync -avizP $(base_name)-$(datestamp).tgz barin:backup/.

semiclean:
	rm -f *~ *.aux *.bbl *.blg *.brf *.bmt *.dvi *.log *.toc \
	$(base_name).pdf $(base_name).ps $(base_name).out $(base_name)Notes.bib

figuresclean:
	$(MAKE) -C figures clean

clean:
	$(MAKE) semiclean

.PHONY: clean figuresclean semiclean backup

